Supporting Proving and Discovering Geometric Inequalities in GeoGebra by using Tarski

We introduce a system of software tools that can automatically prove or discover geometric inequalities. The system, called GeoGebra Discovery, consisting of an extended version of GeoGebra, a controller web service realgeom, and the computational tool Tarski (with the extensive help of the QEPCAD B system) successfully solves several non-trivial problems in Euclidean planar geometry related to inequalities.

==> eptcsdata.tex <==
\providecommand{\firstpage}{156}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.18}{10.4204/EPTCS.352.18}}
\pdfoutput=1

